Occupational mobility network of the Romanian higher education graduates

Although there is a rich literature on the rate of occupational mobility, there are important gaps in understanding patterns of movement among occupations. We employ a network based approach to explore occupational mobility of the Romanian university graduates in the first years after graduation (2003 - 2008). We use survey data on their career mobility to build an empirical occupational mobility network (OMN) that covers all their job movements in the considered period. We construct the network as directed and weighted. The nodes are represented by the occupations (post coded at 3 digits according to ISCO-88) and the links are weighted with the number of persons switching from one occupation to another. This representation of data permits us to use the novel statistical techniques developed in the framework of weighted directed networks in order to extract a set of stylized facts that highlight patterns of occupational mobility: centrality, network motifs.

==> repair.26267.OMN_RO.tex <==
%\begin{filecontents*}{example.eps}


==> repair.26270.Ancona.tex <==
%\begin{filecontents*}{example.eps}


==> repair.26273.OMN_RO.tex <==
%\begin{filecontents*}{example.eps}

